Supersymmetric Configurations, Geometric Transitions and New Non-Kahler Manifolds

We give a detailed derivation of a supersymmetric configuration of wrapped D5-branes on a two-cycle of a warped resolved conifold. Our analysis reveals that the resolved conifold should support a non-Kahler metric with an SU(3) structure. We use this as a starting point of the geometric transition in type IIB theory. A mirror, and a subsequent flop transition using an intermediate M-theory configuration with a G_2 structure, gives rise to the complete IR geometric transition in type IIA theory. A further mirror transformation gives the type IIB gravity dual of the IR gauge theory on the wrapped D5-branes. Expectedly non-Kahler deformations of the resolved and the deformed conifolds appear as the gravity duals of the confining gauge theories in type IIA and type IIB theories respectively, although in more generic cases these manifolds could also be non-geometric. In the local limit we reproduce precisely the scenarios presented in our earlier works. Our present work should therefore be viewed as providing a supergravity proof of geometric transitions in the full global scenarios in type II theories.

==> my.tex <==

\def\blfootnote{\xdef\@thefnmark{}\@footnotetext}

\long\def\symbolfootnote[#1]#2{\begingroup%
\def\thefootnote{\fnsymbol{footnote}}\footnote[#1]{#2}\endgroup}

\def\lsim{ \,\, \vcenter{\hbox{$\buildrel{\displaystyle <}\over\sim$}}
 \,\,}
\def\gsim{ \,\, \vcenter{\hbox{$\buildrel{\displaystyle >}\over\sim$}}
 \,\,}
\def\qeq{ \,\, \vcenter{\hbox{$\buildrel{\displaystyle ?}\over =$}}
 \,\,}
\newcommand{\be}{\begin{eqnarray}}
\newcommand{\ee}{\end{eqnarray}}
\newcommand{\ben}{\begin{eqnarray*}}
\newcommand{\een}{\end{eqnarray*}}
\newcommand{\ampeq}{&=&}
%
% bframe\eframe do not work
%
%\newcommand{\bframe}{\begin{frame}}
%\newcommand{\eframe}{\end{frame}}
%
\newcommand{\bcent}{\begin{center}}
\newcommand{\ecent}{\end{center}}
\newcommand{\benum}{\begin{enumerate}}
\newcommand{\eenum}{\end{enumerate}}
\newcommand{\bdesc}{\begin{description}}
\newcommand{\edesc}{\end{description}}

\newcommand{\parag}[1]{\paragraph{#1}\mbox{}\\ \noindent}

\newcommand{\bitem}{\begin{itemize}}
\newcommand{\eitem}{\end{itemize}}
\newcommand{\setitemsep}[1]{\setlength{\itemsep}{#1}}
\newcommand{\bitemset}[1]{\begin{itemize}\addtolength{\itemsep}{#1}}
\newcommand{\biteml}{\begin{itemize}\addtolength{\itemsep}{+0.1cm}\large}
\newcommand{\bitemL}{\begin{itemize}\addtolength{\itemsep}{+0.1cm}\Large}
\newcommand{\bitemh}{\begin{itemize}\addtolength{\itemsep}{+0.1cm}\huge}
\newcommand{\bitemH}{\begin{itemize}\addtolength{\itemsep}{+0.1cm}\Huge}
\newcommand{\bitemn}{\begin{itemize}\addtolength{\itemsep}{+0.1cm}\normalsize}

\newcommand{\bquote}{\begin{quote}}
\newcommand{\equote}{\end{quote}}
\newcommand{\bhalfp}{\begin{minipage}{0.45\textwidth}}
\newcommand{\ehalfp}{\end{minipage}}
\newcommand{\bhead}{\begin{center}\bf \Large}
\newcommand{\ehead}{\end{center}\bigskip}
\newcommand{\non}{\nonumber\\}
\newcommand{\scrpt}[1]{{\hbox{\scriptsize #1}}}
\newcommand{\mbf}[1]{{\mbox{\boldmath{$#1$}}}}
\newcommand{\inline}[1]{\noalign{\hbox{#1}}}
\newcommand{\colvec}[1]{{\begin{array}{c} #1\end{array}}}
\newcommand{\equ}[1]{Eq.~(\ref{#1})}
% \newcommand{\bbox}[1]{\hbox{\boldmath{$#1$}}}
%
%some vector product short cuts
\newcommand{\dotpr}[2]{{\bf #1}{\cdot}{\bf #2}}
\newcommand{\crosspr}[2]{{\bf #1}{\times}{\bf #2}}
\newcommand{\partiald}[2]{{\partial #1\over \partial #2}}
\newcommand{\partialdif}[1]{{\partial \over \partial #1}}
%
\newcommand{\ul}[1]{\underline{#1}}
%
% math bold faces
%%
 \newcommand{\bfalpha}{{\mbf{\alpha}}}
 \newcommand{\bfbeta}{{\mbf{\beta}}}
 \newcommand{\bfgamma}{{\mbf{\gamma}}}
 \newcommand{\bfdelta}{{\mbf{\delta}}}
 \newcommand{\bfepsilon}{{\mbf{\epsilon}}}
 \newcommand{\bfzeta}{{\mbf{\zeta}}}
 \newcommand{\bfeta}{{\mbf{\eta}}}
 \newcommand{\bftheta}{{\mbf{\theta}}}
 \newcommand{\bfiota}{{\mbf{\iota}}}
 \newcommand{\bfkappa}{{\mbf{\kappa}}}
 \newcommand{\bflambda}{{\mbf{\lambda}}}
 \newcommand{\bfmu}{{\mbf{\mu}}}
 \newcommand{\bfnu}{{\mbf{\nu}}}
 \newcommand{\bfxi}{{\mbf{\xi}}}
% omicron \newcommand{\bfo}{{\mbf{o}}}
 \newcommand{\bfpi}{{\mbf{\pi}}}
 \newcommand{\bfrho}{{\mbf{\rho}}}
 \newcommand{\bfsigma}{{\mbf{\sigma}}}
 \newcommand{\bftau}{{\mbf{\tau}}}
 \newcommand{\bfupsilon}{{\mbf{\upsilon}}}
 \newcommand{\bfphi}{{\mbf{\phi}}}
 \newcommand{\bfvarphi}{{\mbf{\varphi}}}
 \newcommand{\bfchi}{{\mbf{\chi}}}
 \newcommand{\bfpsi}{{\mbf{\psi}}}
 \newcommand{\bfomega}{{\mbf{\omega}}}
 %
 \newcommand{\bfGamma}{{\mbf{\Gamma}}}
 \newcommand{\bfDelta}{{\mbf{\Delta}}}
 \newcommand{\bfTheta}{{\mbf{\Theta}}}
 \newcommand{\bfLambda}{{\mbf{\Lambda}}}
 \newcommand{\bfXi}{{\mbf{\Xi}}}
% omicron \newcommand{\bfo}{{\mbf{o}}}
 \newcommand{\bfPi}{{\mbf{\Pi}}}
 \newcommand{\bfSigma}{{\mbf{\Sigma}}}
 \newcommand{\bfUpsilon}{{\mbf{\Upsilon}}}
 \newcommand{\bfPhi}{{\mbf{\Phi}}}
 \newcommand{\bfPsi}{{\mbf{\Psi}}}
 \newcommand{\bfOmega}{{\mbf{\Omega}}}
%%
%
% bold faces
 \newcommand{\bfa}{{\bf a}} 
 \newcommand{\bfb}{{\bf b}} 
 \newcommand{\bfc}{{\bf c}} 
 \newcommand{\bfd}{{\bf d}} 
 \newcommand{\bfe}{{\bf e}} 
 \newcommand{\bff}{{\bf f}} 
 \newcommand{\bfg}{{\bf g}} 
 \newcommand{\bfh}{{\bf h}} 
 \newcommand{\bfi}{{\bf i}} 
 \newcommand{\bfj}{{\bf j}} 
 \newcommand{\bfk}{{\bf k}} 
 \newcommand{\bfl}{{\bf l}} 
 \newcommand{\bfm}{{\bf m}} 
 \newcommand{\bfn}{{\bf n}} 
 \newcommand{\bfo}{{\bf o}} 
 \newcommand{\bfp}{{\bf p}} 
 \newcommand{\bfq}{{\bf q}} 
 \newcommand{\bfr}{{\bf r}} 
 \newcommand{\bfs}{{\bf s}} 
 \newcommand{\bft}{{\bf t}} 
 \newcommand{\bfu}{{\bf u}} 
 \newcommand{\bfv}{{\bf v}} 
 \newcommand{\bfw}{{\bf w}} 
 \newcommand{\bfx}{{\bf x}} 
 \newcommand{\bfy}{{\bf y}} 
 \newcommand{\bfz}{{\bf z}} 
%
 \newcommand{\bfA}{{\bf A}} 
 \newcommand{\bfB}{{\bf B}} 
 \newcommand{\bfC}{{\bf C}} 
 \newcommand{\bfD}{{\bf D}} 
 \newcommand{\bfE}{{\bf E}} 
 \newcommand{\bfF}{{\bf F}} 
 \newcommand{\bfG}{{\bf G}} 
 \newcommand{\bfH}{{\bf H}} 
 \newcommand{\bfI}{{\bf I}} 
 \newcommand{\bfJ}{{\bf J}} 
 \newcommand{\bfK}{{\bf K}} 
 \newcommand{\bfL}{{\bf L}} 
 \newcommand{\bfM}{{\bf M}} 
 \newcommand{\bfN}{{\bf N}} 
 \newcommand{\bfO}{{\bf O}} 
 \newcommand{\bfP}{{\bf P}} 
 \newcommand{\bfQ}{{\bf Q}} 
 \newcommand{\bfR}{{\bf R}} 
 \newcommand{\bfS}{{\bf S}} 
 \newcommand{\bfT}{{\bf T}} 
 \newcommand{\bfU}{{\bf U}} 
 \newcommand{\bfV}{{\bf V}} 
 \newcommand{\bfW}{{\bf W}} 
 \newcommand{\bfX}{{\bf X}} 
 \newcommand{\bfY}{{\bf Y}} 
 \newcommand{\bfZ}{{\bf Z}} 
%
 \newcommand{\hatbfa}{\hat{\bf a}} 
 \newcommand{\hatbfb}{\hat{\bf b}} 
 \newcommand{\hatbfc}{\hat{\bf c}} 
 \newcommand{\hatbfd}{\hat{\bf d}} 
 \newcommand{\hatbfe}{\hat{\bf e}} 
 \newcommand{\hatbff}{\hat{\bf f}} 
 \newcommand{\hatbfg}{\hat{\bf g}} 
 \newcommand{\hatbfh}{\hat{\bf h}} 
 \newcommand{\hatbfi}{\hat{\bf i}} 
 \newcommand{\hatbfj}{\hat{\bf j}} 
 \newcommand{\hatbfk}{\hat{\bf k}} 
 \newcommand{\hatbfl}{\hat{\bf l}} 
 \newcommand{\hatbfm}{\hat{\bf m}} 
 \newcommand{\hatbfn}{\hat{\bf n}} 
 \newcommand{\hatbfo}{\hat{\bf o}} 
 \newcommand{\hatbfp}{\hat{\bf p}} 
 \newcommand{\hatbfq}{\hat{\bf q}} 
 \newcommand{\hatbfr}{\hat{\bf r}} 
 \newcommand{\hatbfs}{\hat{\bf s}} 
 \newcommand{\hatbft}{\hat{\bf t}} 
 \newcommand{\hatbfu}{\hat{\bf u}} 
 \newcommand{\hatbfv}{\hat{\bf v}} 
 \newcommand{\hatbfw}{\hat{\bf w}} 
 \newcommand{\hatbfx}{\hat{\bf x}} 
 \newcommand{\hatbfy}{\hat{\bf y}} 
 \newcommand{\hatbfz}{\hat{\bf z}} 
%
 \newcommand{\hatbfA}{\hat{\bf A}} 
 \newcommand{\hatbfB}{\hat{\bf B}} 
 \newcommand{\hatbfC}{\hat{\bf C}} 
 \newcommand{\hatbfD}{\hat{\bf D}} 
 \newcommand{\hatbfE}{\hat{\bf E}} 
 \newcommand{\hatbfF}{\hat{\bf F}} 
 \newcommand{\hatbfG}{\hat{\bf G}} 
 \newcommand{\hatbfH}{\hat{\bf H}} 
 \newcommand{\hatbfI}{\hat{\bf I}} 
 \newcommand{\hatbfJ}{\hat{\bf J}} 
 \newcommand{\hatbfK}{\hat{\bf K}} 
 \newcommand{\hatbfL}{\hat{\bf L}} 
 \newcommand{\hatbfM}{\hat{\bf M}} 
 \newcommand{\hatbfN}{\hat{\bf N}} 
 \newcommand{\hatbfO}{\hat{\bf O}} 
 \newcommand{\hatbfP}{\hat{\bf P}} 
 \newcommand{\hatbfQ}{\hat{\bf Q}} 
 \newcommand{\hatbfR}{\hat{\bf R}} 
 \newcommand{\hatbfS}{\hat{\bf S}} 
 \newcommand{\hatbfT}{\hat{\bf T}} 
 \newcommand{\hatbfU}{\hat{\bf U}} 
 \newcommand{\hatbfV}{\hat{\bf V}} 
 \newcommand{\hatbfW}{\hat{\bf W}} 
 \newcommand{\hatbfX}{\hat{\bf X}} 
 \newcommand{\hatbfY}{\hat{\bf Y}} 
 \newcommand{\hatbfZ}{\hat{\bf Z}} 
%
 \newcommand{\hata}{{\hat{a}}}
 \newcommand{\hatb}{{\hat{b}}}
 \newcommand{\hatc}{{\hat{c}}}
 \newcommand{\hatd}{{\hat{d}}}
 \newcommand{\hate}{{\hat{e}}}
 \newcommand{\hatf}{{\hat{f}}}
 \newcommand{\hatg}{{\hat{g}}}
 \newcommand{\hath}{{\hat{h}}}
 \newcommand{\hati}{{\hat{i}}}
 \newcommand{\hatj}{{\hat{j}}}
 \newcommand{\hatk}{{\hat{k}}}
 \newcommand{\hatl}{{\hat{l}}}
 \newcommand{\hatm}{{\hat{m}}}
 \newcommand{\hatn}{{\hat{n}}}
 \newcommand{\hato}{{\hat{o}}}
 \newcommand{\hatp}{{\hat{p}}}
 \newcommand{\hatq}{{\hat{q}}}
 \newcommand{\hatr}{{\hat{r}}}
 \newcommand{\hats}{{\hat{s}}}
 \newcommand{\hatt}{{\hat{t}}}
 \newcommand{\hatu}{{\hat{u}}}
 \newcommand{\hatv}{{\hat{v}}}
 \newcommand{\hatw}{{\hat{w}}}
 \newcommand{\hatx}{{\hat{x}}}
 \newcommand{\haty}{{\hat{y}}}
 \newcommand{\hatz}{{\hat{z}}}
%
 \newcommand{\hatA}{{\hat{A}}}
 \newcommand{\hatB}{{\hat{B}}}
 \newcommand{\hatC}{{\hat{C}}}
 \newcommand{\hatD}{{\hat{D}}}
 \newcommand{\hatE}{{\hat{E}}}
 \newcommand{\hatF}{{\hat{F}}}
 \newcommand{\hatG}{{\hat{G}}}
 \newcommand{\hatH}{{\hat{H}}}
 \newcommand{\hatI}{{\hat{I}}}
 \newcommand{\hatJ}{{\hat{J}}}
 \newcommand{\hatK}{{\hat{K}}}
 \newcommand{\hatL}{{\hat{L}}}
 \newcommand{\hatM}{{\hat{M}}}
 \newcommand{\hatN}{{\hat{N}}}
 \newcommand{\hatO}{{\hat{O}}}
 \newcommand{\hatP}{{\hat{P}}}
 \newcommand{\hatQ}{{\hat{Q}}}
 \newcommand{\hatR}{{\hat{R}}}
 \newcommand{\hatS}{{\hat{S}}}
 \newcommand{\hatT}{{\hat{T}}}
 \newcommand{\hatU}{{\hat{U}}}
 \newcommand{\hatV}{{\hat{V}}}
 \newcommand{\hatW}{{\hat{W}}}
 \newcommand{\hatX}{{\hat{X}}}
 \newcommand{\hatY}{{\hat{Y}}}
 \newcommand{\hatZ}{{\hat{Z}}}
%
 \newcommand{\hatalpha}{{\hat{\alpha}}}
 \newcommand{\hatbeta}{{\hat{\beta}}}
 \newcommand{\hatgamma}{{\hat{\gamma}}}
 \newcommand{\hatdelta}{{\hat{\delta}}}
 \newcommand{\hatepsilon}{{\hat{\epsilon}}}
 \newcommand{\hatzeta}{{\hat{\zeta}}}
 \newcommand{\hateta}{{\hat{\eta}}}
 \newcommand{\hattheta}{{\hat{\theta}}}
 \newcommand{\hatiota}{{\hat{\iota}}}
 \newcommand{\hatkappa}{{\hat{\kappa}}}
 \newcommand{\hatlambda}{{\hat{\lambda}}}
 \newcommand{\hatmu}{{\hat{\mu}}}
 \newcommand{\hatnu}{{\hat{\nu}}}
 \newcommand{\hatxi}{{\hat{\xi}}}
% omicron \newcommand{\hato}{{\hat{o}}}
 \newcommand{\hatpi}{{\hat{\pi}}}
 \newcommand{\hatrho}{{\hat{\rho}}}
 \newcommand{\hatsigma}{{\hat{\sigma}}}
 \newcommand{\hattau}{{\hat{\tau}}}
 \newcommand{\hatupsilon}{{\hat{\upsilon}}}
 \newcommand{\hatphi}{{\hat{\phi}}}
 \newcommand{\hatvarphi}{{\hat{\varphi}}}
 \newcommand{\hatchi}{{\hat{\chi}}}
 \newcommand{\hatpsi}{{\hat{\psi}}}
 \newcommand{\hatomega}{{\hat{\omega}}}
 %
 \newcommand{\hatGamma}{{\hat{\Gamma}}}
 \newcommand{\hatDelta}{{\hat{\Delta}}}
 \newcommand{\hatTheta}{{\hat{\Theta}}}
 \newcommand{\hatLambda}{{\hat{\Lambda}}}
 \newcommand{\hatXi}{{\hat{\Xi}}}
% omicron \newcommand{\hato}{{\hat{o}}}
 \newcommand{\hatPi}{{\hat{\Pi}}}
 \newcommand{\hatSigma}{{\hat{\Sigma}}}
 \newcommand{\hatUpsilon}{{\hat{\Upsilon}}}
 \newcommand{\hatPhi}{{\hat{\Phi}}}
 \newcommand{\hatPsi}{{\hat{\Psi}}}
 \newcommand{\hatOmega}{{\hat{\Omega}}}
%
%
 \newcommand{\veca}{{\vec{a}}}
 \newcommand{\vecb}{{\vec{b}}}
 \newcommand{\vecc}{{\vec{c}}}
 \newcommand{\vecd}{{\vec{d}}}
 \newcommand{\vece}{{\vec{e}}}
 \newcommand{\vecf}{{\vec{f}}}
 \newcommand{\vecg}{{\vec{g}}}
 \newcommand{\vech}{{\vec{h}}}
 \newcommand{\veci}{{\vec{i}}}
 \newcommand{\vecj}{{\vec{j}}}
 \newcommand{\veck}{{\vec{k}}}
 \newcommand{\vecl}{{\vec{l}}}
 \newcommand{\vecm}{{\vec{m}}}
 \newcommand{\vecn}{{\vec{n}}}
 \newcommand{\veco}{{\vec{o}}}
 \newcommand{\vecp}{{\vec{p}}}
 \newcommand{\vecq}{{\vec{q}}}
 \newcommand{\vecr}{{\vec{r}}}
 \newcommand{\vecs}{{\vec{s}}}
 \newcommand{\vect}{{\vec{t}}}
 \newcommand{\vecu}{{\vec{u}}}
 \newcommand{\vecv}{{\vec{v}}}
 \newcommand{\vecw}{{\vec{w}}}
 \newcommand{\vecx}{{\vec{x}}}
 \newcommand{\vecy}{{\vec{y}}}
 \newcommand{\vecz}{{\vec{z}}}
%
 \newcommand{\vecA}{{\vec{A}}}
 \newcommand{\vecB}{{\vec{B}}}
 \newcommand{\vecC}{{\vec{C}}}
 \newcommand{\vecD}{{\vec{D}}}
 \newcommand{\vecE}{{\vec{E}}}
 \newcommand{\vecF}{{\vec{F}}}
 \newcommand{\vecG}{{\vec{G}}}
 \newcommand{\vecH}{{\vec{H}}}
 \newcommand{\vecI}{{\vec{I}}}
 \newcommand{\vecJ}{{\vec{J}}}
 \newcommand{\vecK}{{\vec{K}}}
 \newcommand{\vecL}{{\vec{L}}}
 \newcommand{\vecM}{{\vec{M}}}
 \newcommand{\vecN}{{\vec{N}}}
 \newcommand{\vecO}{{\vec{O}}}
 \newcommand{\vecP}{{\vec{P}}}
 \newcommand{\vecQ}{{\vec{Q}}}
 \newcommand{\vecR}{{\vec{R}}}
 \newcommand{\vecS}{{\vec{S}}}
 \newcommand{\vecT}{{\vec{T}}}
 \newcommand{\vecU}{{\vec{U}}}
 \newcommand{\vecV}{{\vec{V}}}
 \newcommand{\vecW}{{\vec{W}}}
 \newcommand{\vecX}{{\vec{X}}}
 \newcommand{\vecY}{{\vec{Y}}}
 \newcommand{\vecZ}{{\vec{Z}}}
%
 \newcommand{\vecalpha}{{\vec{\alpha}}}
 \newcommand{\vecbeta}{{\vec{\beta}}}
 \newcommand{\vecgamma}{{\vec{\gamma}}}
 \newcommand{\vecdelta}{{\vec{\delta}}}
 \newcommand{\vecepsilon}{{\vec{\epsilon}}}
 \newcommand{\veczeta}{{\vec{\zeta}}}
 \newcommand{\veceta}{{\vec{\eta}}}
 \newcommand{\vectheta}{{\vec{\theta}}}
 \newcommand{\veciota}{{\vec{\iota}}}
 \newcommand{\veckappa}{{\vec{\kappa}}}
 \newcommand{\veclambda}{{\vec{\lambda}}}
 \newcommand{\vecmu}{{\vec{\mu}}}
 \newcommand{\vecnu}{{\vec{\nu}}}
 \newcommand{\vecxi}{{\vec{\xi}}}
% omicron \newcommand{\veco}{{\vec{o}}}
 \newcommand{\vecpi}{{\vec{\pi}}}
 \newcommand{\vecrho}{{\vec{\rho}}}
 \newcommand{\vecsigma}{{\vec{\sigma}}}
 \newcommand{\vectau}{{\vec{\tau}}}
 \newcommand{\vecupsilon}{{\vec{\upsilon}}}
 \newcommand{\vecphi}{{\vec{\phi}}}
 \newcommand{\vecvarphi}{{\vec{\varphi}}}
 \newcommand{\vecchi}{{\vec{\chi}}}
 \newcommand{\vecpsi}{{\vec{\psi}}}
 \newcommand{\vecomega}{{\vec{\omega}}}
 %
 \newcommand{\vecGamma}{{\vec{\Gamma}}}
 \newcommand{\vecDelta}{{\vec{\Delta}}}
 \newcommand{\vecTheta}{{\vec{\Theta}}}
 \newcommand{\vecLambda}{{\vec{\Lambda}}}
 \newcommand{\vecXi}{{\vec{\Xi}}}
% omicron \newcommand{\veco}{{\vec{o}}}
 \newcommand{\vecPi}{{\vec{\Pi}}}
 \newcommand{\vecSigma}{{\vec{\Sigma}}}
 \newcommand{\vecUpsilon}{{\vec{\Upsilon}}}
 \newcommand{\vecPhi}{{\vec{\Phi}}}
 \newcommand{\vecPsi}{{\vec{\Psi}}}
 \newcommand{\vecOmega}{{\vec{\Omega}}}
%%%%%%%%
 \newcommand{\tildea}{{\tilde{a}}}
 \newcommand{\tildeb}{{\tilde{b}}}
 \newcommand{\tildec}{{\tilde{c}}}
 \newcommand{\tilded}{{\tilde{d}}}
 \newcommand{\tildee}{{\tilde{e}}}
 \newcommand{\tildef}{{\tilde{f}}}
 \newcommand{\tildeg}{{\tilde{g}}}
 \newcommand{\tildeh}{{\tilde{h}}}
 \newcommand{\tildei}{{\tilde{i}}}
 \newcommand{\tildej}{{\tilde{j}}}
 \newcommand{\tildek}{{\tilde{k}}}
 \newcommand{\tildel}{{\tilde{l}}}
 \newcommand{\tildem}{{\tilde{m}}}
 \newcommand{\tilden}{{\tilde{n}}}
 \newcommand{\tildeo}{{\tilde{o}}}
 \newcommand{\tildep}{{\tilde{p}}}
 \newcommand{\tildeq}{{\tilde{q}}}
 \newcommand{\tilder}{{\tilde{r}}}
 \newcommand{\tildes}{{\tilde{s}}}
 \newcommand{\tildet}{{\tilde{t}}}
 \newcommand{\tildeu}{{\tilde{u}}}
 \newcommand{\tildev}{{\tilde{v}}}
 \newcommand{\tildew}{{\tilde{w}}}
 \newcommand{\tildex}{{\tilde{x}}}
 \newcommand{\tildey}{{\tilde{y}}}
 \newcommand{\tildez}{{\tilde{z}}}
%
 \newcommand{\tildeA}{{\tilde{A}}}
 \newcommand{\tildeB}{{\tilde{B}}}
 \newcommand{\tildeC}{{\tilde{C}}}
 \newcommand{\tildeD}{{\tilde{D}}}
 \newcommand{\tildeE}{{\tilde{E}}}
 \newcommand{\tildeF}{{\tilde{F}}}
 \newcommand{\tildeG}{{\tilde{G}}}
 \newcommand{\tildeH}{{\tilde{H}}}
 \newcommand{\tildeI}{{\tilde{I}}}
 \newcommand{\tildeJ}{{\tilde{J}}}
 \newcommand{\tildeK}{{\tilde{K}}}
 \newcommand{\tildeL}{{\tilde{L}}}
 \newcommand{\tildeM}{{\tilde{M}}}
 \newcommand{\tildeN}{{\tilde{N}}}
 \newcommand{\tildeO}{{\tilde{O}}}
 \newcommand{\tildeP}{{\tilde{P}}}
 \newcommand{\tildeQ}{{\tilde{Q}}}
 \newcommand{\tildeR}{{\tilde{R}}}
 \newcommand{\tildeS}{{\tilde{S}}}
 \newcommand{\tildeT}{{\tilde{T}}}
 \newcommand{\tildeU}{{\tilde{U}}}
 \newcommand{\tildeV}{{\tilde{V}}}
 \newcommand{\tildeW}{{\tilde{W}}}
 \newcommand{\tildeX}{{\tilde{X}}}
 \newcommand{\tildeY}{{\tilde{Y}}}
 \newcommand{\tildeZ}{{\tilde{Z}}}
%
 \newcommand{\tildealpha}{{\tilde{\alpha}}}
 \newcommand{\tildebeta}{{\tilde{\beta}}}
 \newcommand{\tildegamma}{{\tilde{\gamma}}}
 \newcommand{\tildedelta}{{\tilde{\delta}}}
 \newcommand{\tildeepsilon}{{\tilde{\epsilon}}}
 \newcommand{\tildezeta}{{\tilde{\zeta}}}
 \newcommand{\tildeeta}{{\tilde{\eta}}}
 \newcommand{\tildetheta}{{\tilde{\theta}}}
 \newcommand{\tildeiota}{{\tilde{\iota}}}
 \newcommand{\tildekappa}{{\tilde{\kappa}}}
 \newcommand{\tildelambda}{{\tilde{\lambda}}}
 \newcommand{\tildemu}{{\tilde{\mu}}}
 \newcommand{\tildenu}{{\tilde{\nu}}}
 \newcommand{\tildexi}{{\tilde{\xi}}}
% omicron \newcommand{\tildeo}{{\tilde{o}}}
 \newcommand{\tildepi}{{\tilde{\pi}}}
 \newcommand{\tilderho}{{\tilde{\rho}}}
 \newcommand{\tildesigma}{{\tilde{\sigma}}}
 \newcommand{\tildetau}{{\tilde{\tau}}}
 \newcommand{\tildeupsilon}{{\tilde{\upsilon}}}
 \newcommand{\tildephi}{{\tilde{\phi}}}
 \newcommand{\tildevarphi}{{\tilde{\varphi}}}
 \newcommand{\tildechi}{{\tilde{\chi}}}
 \newcommand{\tildepsi}{{\tilde{\psi}}}
 \newcommand{\tildeomega}{{\tilde{\omega}}}
 %
 \newcommand{\tildeGamma}{{\tilde{\Gamma}}}
 \newcommand{\tildeDelta}{{\tilde{\Delta}}}
 \newcommand{\tildeTheta}{{\tilde{\Theta}}}
 \newcommand{\tildeLambda}{{\tilde{\Lambda}}}
 \newcommand{\tildeXi}{{\tilde{\Xi}}}
% omicron \newcommand{\tildeo}{{\tilde{o}}}
 \newcommand{\tildePi}{{\tilde{\Pi}}}
 \newcommand{\tildeSigma}{{\tilde{\Sigma}}}
 \newcommand{\tildeUpsilon}{{\tilde{\Upsilon}}}
 \newcommand{\tildePhi}{{\tilde{\Phi}}}
 \newcommand{\tildePsi}{{\tilde{\Psi}}}
 \newcommand{\tildeOmega}{{\tilde{\Omega}}}
%
 \newcommand{\tildepartial}{{\tilde{\partial}}}
%%
%%
 \newcommand{\bara}{{\bar{a}}}
 \newcommand{\barb}{{\bar{b}}}
 \newcommand{\barc}{{\bar{c}}}
 \newcommand{\bard}{{\bar{d}}}
 \newcommand{\bare}{{\bar{e}}}
 \newcommand{\barf}{{\bar{f}}}
 \newcommand{\barg}{{\bar{g}}}
 \newcommand{\barh}{{\bar{h}}}
 \newcommand{\bari}{{\bar{i}}}
 \newcommand{\barj}{{\bar{j}}}
 \newcommand{\bark}{{\bar{k}}}
 \newcommand{\barl}{{\bar{l}}}
 \newcommand{\barm}{{\bar{m}}}
 \newcommand{\barn}{{\bar{n}}}
 \newcommand{\baro}{{\bar{o}}}
 \newcommand{\barp}{{\bar{p}}}
 \newcommand{\barq}{{\bar{q}}}
 \newcommand{\barr}{{\bar{r}}}
 \newcommand{\bars}{{\bar{s}}}
 \newcommand{\bart}{{\bar{t}}}
 \newcommand{\baru}{{\bar{u}}}
 \newcommand{\barv}{{\bar{v}}}
 \newcommand{\barw}{{\bar{w}}}
 \newcommand{\barx}{{\bar{x}}}
 \newcommand{\bary}{{\bar{y}}}
 \newcommand{\barz}{{\bar{z}}}
%
 \newcommand{\barA}{{\bar{A}}}
 \newcommand{\barB}{{\bar{B}}}
 \newcommand{\barC}{{\bar{C}}}
 \newcommand{\barD}{{\bar{D}}}
 \newcommand{\barE}{{\bar{E}}}
 \newcommand{\barF}{{\bar{F}}}
 \newcommand{\barG}{{\bar{G}}}
 \newcommand{\barH}{{\bar{H}}}
 \newcommand{\barI}{{\bar{I}}}
 \newcommand{\barJ}{{\bar{J}}}
 \newcommand{\barK}{{\bar{K}}}
 \newcommand{\barL}{{\bar{L}}}
 \newcommand{\barM}{{\bar{M}}}
 \newcommand{\barN}{{\bar{N}}}
 \newcommand{\barO}{{\bar{O}}}
 \newcommand{\barP}{{\bar{P}}}
 \newcommand{\barQ}{{\bar{Q}}}
 \newcommand{\barR}{{\bar{R}}}
 \newcommand{\barS}{{\bar{S}}}
 \newcommand{\barT}{{\bar{T}}}
 \newcommand{\barU}{{\bar{U}}}
 \newcommand{\barV}{{\bar{V}}}
 \newcommand{\barW}{{\bar{W}}}
 \newcommand{\barX}{{\bar{X}}}
 \newcommand{\barY}{{\bar{Y}}}
 \newcommand{\barZ}{{\bar{Z}}}
%
 \newcommand{\baralpha}{{\bar{\alpha}}}
 \newcommand{\barbeta}{{\bar{\beta}}}
 \newcommand{\bargamma}{{\bar{\gamma}}}
 \newcommand{\bardelta}{{\bar{\delta}}}
 \newcommand{\barepsilon}{{\bar{\epsilon}}}
 \newcommand{\barzeta}{{\bar{\zeta}}}
 \newcommand{\bareta}{{\bar{\eta}}}
 \newcommand{\bartheta}{{\bar{\theta}}}
 \newcommand{\bariota}{{\bar{\iota}}}
 \newcommand{\barkappa}{{\bar{\kappa}}}
 \newcommand{\barlambda}{{\bar{\lambda}}}
 \newcommand{\barmu}{{\bar{\mu}}}
 \newcommand{\barnu}{{\bar{\nu}}}
 \newcommand{\barxi}{{\bar{\xi}}}
% omicron \newcommand{\baro}{{\bar{o}}}
 \newcommand{\barpi}{{\bar{\pi}}}
 \newcommand{\barrho}{{\bar{\rho}}}
 \newcommand{\barsigma}{{\bar{\sigma}}}
 \newcommand{\bartau}{{\bar{\tau}}}
 \newcommand{\barupsilon}{{\bar{\upsilon}}}
 \newcommand{\barphi}{{\bar{\phi}}}
 \newcommand{\barvarphi}{{\bar{\varphi}}}
 \newcommand{\barchi}{{\bar{\chi}}}
 \newcommand{\barpsi}{{\bar{\psi}}}
 \newcommand{\baromega}{{\bar{\omega}}}
 %
 \newcommand{\barGamma}{{\bar{\Gamma}}}
 \newcommand{\barDelta}{{\bar{\Delta}}}
 \newcommand{\barTheta}{{\bar{\Theta}}}
 \newcommand{\barLambda}{{\bar{\Lambda}}}
 \newcommand{\barXi}{{\bar{\Xi}}}
% omicron \newcommand{\baro}{{\bar{o}}}
 \newcommand{\barPi}{{\bar{\Pi}}}
 \newcommand{\barSigma}{{\bar{\Sigma}}}
 \newcommand{\barUpsilon}{{\bar{\Upsilon}}}
 \newcommand{\barPhi}{{\bar{\Phi}}}
 \newcommand{\barPsi}{{\bar{\Psi}}}
 \newcommand{\barOmega}{{\bar{\Omega}}}
%%
%math bolds
 \newcommand{\mbfa}{{\mbf{a}}}
 \newcommand{\mbfb}{{\mbf{b}}}
 \newcommand{\mbfc}{{\mbf{c}}}
 \newcommand{\mbfd}{{\mbf{d}}}
 \newcommand{\mbfe}{{\mbf{e}}}
 \newcommand{\mbff}{{\mbf{f}}}
 \newcommand{\mbfg}{{\mbf{g}}}
 \newcommand{\mbfh}{{\mbf{h}}}
 \newcommand{\mbfi}{{\mbf{i}}}
 \newcommand{\mbfj}{{\mbf{j}}}
 \newcommand{\mbfk}{{\mbf{k}}}
 \newcommand{\mbfl}{{\mbf{l}}}
 \newcommand{\mbfm}{{\mbf{m}}}
 \newcommand{\mbfn}{{\mbf{n}}}
 \newcommand{\mbfo}{{\mbf{o}}}
 \newcommand{\mbfp}{{\mbf{p}}}
 \newcommand{\mbfq}{{\mbf{q}}}
 \newcommand{\mbfr}{{\mbf{r}}}
 \newcommand{\mbfs}{{\mbf{s}}}
 \newcommand{\mbft}{{\mbf{t}}}
 \newcommand{\mbfu}{{\mbf{u}}}
 \newcommand{\mbfv}{{\mbf{v}}}
 \newcommand{\mbfw}{{\mbf{w}}}
 \newcommand{\mbfx}{{\mbf{x}}}
 \newcommand{\mbfy}{{\mbf{y}}}
 \newcommand{\mbfz}{{\mbf{z}}}
%
 \newcommand{\mbfA}{{\mbf{A}}}
 \newcommand{\mbfB}{{\mbf{B}}}
 \newcommand{\mbfC}{{\mbf{C}}}
 \newcommand{\mbfD}{{\mbf{D}}}
 \newcommand{\mbfE}{{\mbf{E}}}
 \newcommand{\mbfF}{{\mbf{F}}}
 \newcommand{\mbfG}{{\mbf{G}}}
 \newcommand{\mbfH}{{\mbf{H}}}
 \newcommand{\mbfI}{{\mbf{I}}}
 \newcommand{\mbfJ}{{\mbf{J}}}
 \newcommand{\mbfK}{{\mbf{K}}}
 \newcommand{\mbfL}{{\mbf{L}}}
 \newcommand{\mbfM}{{\mbf{M}}}
 \newcommand{\mbfN}{{\mbf{N}}}
 \newcommand{\mbfO}{{\mbf{O}}}
 \newcommand{\mbfP}{{\mbf{P}}}
 \newcommand{\mbfQ}{{\mbf{Q}}}
 \newcommand{\mbfR}{{\mbf{R}}}
 \newcommand{\mbfS}{{\mbf{S}}}
 \newcommand{\mbfT}{{\mbf{T}}}
 \newcommand{\mbfU}{{\mbf{U}}}
 \newcommand{\mbfV}{{\mbf{V}}}
 \newcommand{\mbfW}{{\mbf{W}}}
 \newcommand{\mbfX}{{\mbf{X}}}
 \newcommand{\mbfY}{{\mbf{Y}}}
 \newcommand{\mbfZ}{{\mbf{Z}}}
%
 \newcommand{\calA}{{\cal A}}
 \newcommand{\calB}{{\cal B}}
 \newcommand{\calC}{{\cal C}}
 \newcommand{\calD}{{\cal D}}
 \newcommand{\calE}{{\cal E}}
 \newcommand{\calF}{{\cal F}}
 \newcommand{\calG}{{\cal G}}
 \newcommand{\calH}{{\cal H}}
 \newcommand{\calI}{{\cal I}}
 \newcommand{\calJ}{{\cal J}}
 \newcommand{\calK}{{\cal K}}
 \newcommand{\calL}{{\cal L}}
 \newcommand{\calM}{{\cal M}}
 \newcommand{\calN}{{\cal N}}
 \newcommand{\calO}{{\cal O}}
 \newcommand{\calP}{{\cal P}}
 \newcommand{\calQ}{{\cal Q}}
 \newcommand{\calR}{{\cal R}}
 \newcommand{\calS}{{\cal S}}
 \newcommand{\calT}{{\cal T}}
 \newcommand{\calU}{{\cal U}}
 \newcommand{\calV}{{\cal V}}
 \newcommand{\calW}{{\cal W}}
 \newcommand{\calX}{{\cal X}}
 \newcommand{\calY}{{\cal Y}}
 \newcommand{\calZ}{{\cal Z}}
%
 \newcommand{\hbarc}{(\hbar c)}
 \newcommand{\dmom}[1]{{d^3 #1 \over (2\pi)^3}}
 \newcommand{\ddmom}[2]{{d^{#1} #2 \over (2\pi)^{#1}}}
 \newcommand{\dphase}[1]{{d^3 #1 \over (2\pi)^3 2E_{#1}}}
 \newcommand{\dom}[1]{{d #1 \over 2\pi}}
 \newcommand{\dum}{{\vphantom{x}}} 
 \newcommand{\Tr}{{\rm Tr}}
 \newcommand{\Det}{{\rm Det}\,}
 \newcommand{\qave}[1]{\left\langle {#1} \right\rangle}
 \newcommand{\sandwich}[3]{\left\langle{#1}\left|{#2}\right|{#3}\right\rangle}
 \newcommand{\absol}[1]{\left| #1 \right|}
 \newcommand{\eqn}[1]{Eq.~(\ref{#1})}
 \newcommand{\heading}[1]{\bigskip\noindent{\bf #1}\\}
 \newcommand{\bra}[1]{\langle {#1} |}
 \newcommand{\ket}[1]{| {#1} \rangle}
 \newcommand{\braket}[2]{
              \left\langle
	      \left. {#1} \vphantom{#1} \vphantom{#2} \right|
	      {#2}\right\rangle}
 \newcommand{\ketbra}[2]{
              \left| {#1} \vphantom{#1} \vphantom{#2} \right\rangle
	      \left\langle {#2}\right|}
 \newcommand{\intinfty}{\int_{-\infty}^{\infty}}
 \newcommand{\sumint}{\sum\hspace{-0.5cm}\int}
 \newcommand{\ave}[1]{\langle {#1} \rangle}
 \newcommand{\up}{\uparrow}
 \newcommand{\down}{\downarrow}
% length units
\newcommand{\meter}{\hbox{m}}
\newcommand{\fm}{\hbox{fm}}
\newcommand{\picom}{\hbox{pm}}
\newcommand{\nm}{\hbox{nm}}
\newcommand{\microm}{{\mu\hbox{m}}}
\newcommand{\mm}{\hbox{mm}}
\newcommand{\cm}{\hbox{cm}}
\newcommand{\km}{\hbox{km}}
\newcommand{\mb}{\hbox{mb}}
%
%energy units
%
\newcommand{\Joule}{\hbox{J}}
\newcommand{\TeV}{\hbox{TeV}}
\newcommand{\GeV}{\hbox{GeV}}
\newcommand{\MeV}{\hbox{MeV}}
\newcommand{\keV}{\hbox{keV}}
\newcommand{\eV}{\hbox{eV}}
\newcommand{\meV}{\hbox{meV}}
% 
%frequency units
%
\newcommand{\THz}{\hbox{THz}}
\newcommand{\GHz}{\hbox{GHz}}
\newcommand{\MHz}{\hbox{MHz}}
\newcommand{\kHz}{\hbox{kHz}}
\newcommand{\Hz}{\hbox{Hz}}
%
\newcommand{\gram}{\hbox{g}}
\newcommand{\kg}{\hbox{kg}}
\newcommand{\newton}{\hbox{N}}

\newcommand{\red}{\color{red}}
\newcommand{\blue}{\color{blue}}
\newcommand{\green}{\color{green}}
\newcommand{\magenta}{\color{magenta}}
\newcommand{\cyan}{\color{cyan}}
\newcommand{\yellow}{\color{yellow}}
\newcommand{\black}{\color{black}}
\newcommand{\white}{\color{white}}
%

\newcommand{\Nch}{N_{\rm ch}}
\newcommand{\mth}{m_{\rm th}}

%
 \newcommand{\eq}[1]{{$\displaystyle #1$}}
 \newcommand{\tw}{\textwidth}
 \newcommand{\fig}[2]{\bigskip\psfig{figure=#1,width=#2\textwidth}\bigskip}
% mathematica stuff
 \newcommand{\Mvariable}[1]{#1}
 \newcommand{\Mfunction}[1]{{\hbox{#1}}}
 \newcommand{\Muserfunction}[1]{{\hbox{#1}}}
 \newcommand{\imag}{i}
%
\newcommand{\bang}[1]{\textbf{#1}}
\newcommand{\showbf}[1]{\begin{center}{\bf #1}\end{center}}
\newcommand{\degC}{{}^\circ{\rm C}}
\newcommand{\degK}{{\rm K}}
\newcommand{\putfig}[4]{
 \begin{figure}[h!]
  \epsfxsize=#1
  \centerline{\epsfbox{#2}}
  \caption{#3}
  \label{#4}
 \end{figure}}
\newcommand{\microstate}{{\bf micro}state\ }
\newcommand{\microstates}{{\bf micro}states\ }
\newcommand{\macrostate}{{\bf macro}state\ }
\newcommand{\macrostates}{{\bf macro}states\ }
%
% Guy'd defs
\newcommand{\h}{{\bf h}}
\newcommand{\p}{{\bf p}}
\newcommand{\q}{{\bf q}}
\newcommand{\F}{{\bf F}}
\newcommand{\gs}{g_{\rm s}}
\newcommand{\Pg}{P_{g}}
\newcommand{\Pq}{P_{q\bar{q}}}

\newcommand{\twobytwo}[4]
{\left(\begin{array}{cc}#1 & #2 \\ #3 & #4\end{array}\right)}

\newcommand{\bmat}[1]{\left(\begin{array}{#1}}
\newcommand{\emat}{\end{array}\right)}

%%%%%%%%%%%%%%%%%%%%

\usepackage{graphicx}
%this is somehow needed to fix the paper size to letter

